On the Role of Contrast and Regularity in Perceptual Boundary Saliency

Mathematical Morphology proposes to extract shapes from images as connected components of level sets. These methods prove very suitable for shape recognition and analysis. We present a method to select the perceptually significant (i.e., contrasted) level lines (boundaries of level sets), using the Helmholtz principle as first proposed by Desolneux et al. Contrarily to the classical formulation by Desolneux et al. where level lines must be entirely salient, the proposed method allows to detect partially salient level lines, thus resulting in more robust and more stable detections. We then tackle the problem of combining two gestalts as a measure of saliency and propose a method that reinforces detections. Results in natural images show the good performance of the proposed methods.

==> meaningful boundaries preprint/proofNFA_C.tex <==
\subsection{Meaningful Contrasted Boundaries}
\label{sec:proofNFA_C}

This section proves that TMA-MCB (see Definition~\ref{def:nfaContrastedCurve_k}, p.~\pageref{def:nfaContrastedCurve_k}) are theoretically correct.
As usual, being correct means that the following proposition holds.
\begin{proposition}
  The expected number of TMA \meps-meaningful boundaries in a finite set $E$ of random curves is smaller than \meps.
\end{proposition}

\begin{proof}
  For this proof we follow the scheme from Proposition~12 in~\cite{cao08theory}.

  For all $k$, let us denote by $L_k$ the random length of the pieces of $C$ such that $|Du| \geq \mu_k$. From Definition~\ref{def:nfaContrastedCurve_k}, any curve $C$ is \meps-meaningful if there is at least one $0 \leq k < K$ such that
%  $N_{ll} \ K \ I (H_c(\mu_k); L_1^k, l_2 (k)) < \eps$.
  $N_{ll} \ K \ \widetilde{\bintail} (n \cdot \lsn{2}, L_k; H_c(\mu_k)) < \eps$.
  Let us denote by $E(C, k)$ this event and recall that all probabilities are under $\Hy_0$:
%  \begin{equation*}
%    \Pr (E(C, k)) \stackrel{\mathrm{def}}{=} \Pr (I(Hc(\mu_k); X; l_2(k, 2)) < \frac{\eps}{N_{ll} \ K})
%  \end{equation*}
  \begin{equation*}
    \Pr (E(C, k)) \stackrel{\mathrm{def}}{=} \Pr \left( \widetilde{\bintail} (n \cdot \lsn{2}, L_k; H_c(\mu_k) < \frac{\eps}{N_{ll} \ K} \right) \text{.}
  \end{equation*}

  From Lemma~\ref{lem:classic}, we denote
%  \begin{align*}
%    X & = L_k  & S(x) & = I(Hc(\mu_k); x; l_2(k, 2)) \\
%    t & = \frac{\eps}{N_{ll} \ K} &\quad \Pr(S(X) <  t) & =  \Pr (E(C, k))
%  \end{align*}
  \begin{align*}
    X & = L_k  & S(x) & = \widetilde{\bintail} (n \cdot \lsn{2}, x; Hc(\mu_k)) \\
    t & = \frac{\eps}{N_{ll} \ K} &\quad \Pr(S(X) <  t) & =  \Pr (E(C, k))
  \end{align*}
  and finally
  \begin{equation*}
    \Pr (E(C, k)) \leq \frac{\eps}{N_{ll} \cdot K} \text{.}
  \end{equation*}

  The event defined by ``C is \meps-meaningful'' is $$E(C) = \bigcup_{0 \leq k < K} E(C, k).$$ Let us denote by $\expectation_{\Hy_0}$ the mathematical expectation under $\Hy_0$. The expected number of \meps-meaningful curves is defined as $\mathbb{E}_{\Hy_0} \left( \sum_{C \in \mathcal{C}} \mathbf{1}_{E(C)} \right)$ where $\mathbf{1}_{A}$ is the indicator function of the set $A$.
  Then
  \begin{equation*}
    \expectation_{\Hy_0} \left( \sum_{C \in \mathcal{C}} \mathbf{1}_{E(C)} \right) \leq \sum_{\substack{ C \in \mathcal{C} \\ 0 \leq k < K }} \Pr \left( E(C, k) \right)
    \leq \sum_{\substack{C \in \mathcal{C} \\ 0 \leq k < K}} \frac{\eps}{N_{ll} \cdot K} = \eps.
  \end{equation*}

\end{proof}

==> meaningful boundaries preprint/proofNFA_CR.tex <==
\subsection{Meaningful Contrasted Regular Boundaries}
\label{sec:proofNFA_CR}


%We now prove the theoretically corectness of TMA meaningful contrasted regular boundaries (see Definition~\ref{def:nfaContrastedSmoothCurve_k}, p.~\pageref{def:nfaContrastedSmoothCurve_k}).
%Let us recall the equation in Definition~\ref{def:nfaContrastedSmoothCurve_k}:
%\begin{equation*}
%  \NFA_K^{\mathrm{CR}}(C) \stackrel{\mathrm{def}}{=} N_{ll}\ K_c\ K_s
%  \max \left(
%  \begin{split}
%  \min_{0 \leq k < K_c}I_c (C, k)^2 \\
%  \min_{0 \leq k' < K_s} I_s (C, k')^2
%  \end{split}
%  \right) \text{.}
%  \label{eq:nfaContrastedSmoothCurve_k}
%\end{equation*}
TMA \meps-meaningful boundaries (see Definition~\ref{def:nfaContrastedSmoothCurve_k}, p.~\pageref{def:nfaContrastedSmoothCurve_k}) are correct is the following proposition holds.
\begin{proposition}
  The expected number of \meps-meaningful contrasted regular boundaries, obtained with Definition~\ref{def:nfaContrastedSmoothCurve_k}, in a finite random set $E$ of random curves is smaller than \meps.
\end{proposition}

\begin{proof}
  The same assumptions from the previous proof hold.
  
  Let $X_i = \mathbf{1}_{C_i \mathrm{\ is\ meaningful}}$ and $N = \#E$. Let us denote by $\expectation_{\Hy_0}$ the mathematical expectation under $\Hy_0$. Then
  \begin{multline}
    \expectation \left( \sum_{i=1}^{N} \sum_{k=1}^{K_c} \sum_{k'=1}^{K_s} X_i \right) = \\ \expectation \left( \expectation \left( \sum_{i=1}^{n} \sum_{k=1}^{k_c} \sum_{k'=1}^{k_s} X_i \ |\ N = n, K_c = k_c, K_s = k_s \right) \right) \textbf{.}
  \end{multline}
  We have assumed that $N$ is independent from the curves and $K_c$, $K_s$ are input parameters. Thus, conditionally to $N = n$, the law of $\sum_{i=1}^{N} X_i$ is the law of $\sum_{i=1}^{n} Y_i$ where 
    $$ \displaystyle Y_i = \mathbf{1}_{n\, k_c\, k_s\, \max \left(\min_{0 \leq k < k_c}I_c (C_i, k)^2,\  \min_{0 \leq k' < k_s} I_s (C_i, k')^2 \right)  < \eps}. $$
  By the linearity of expectation
  \begin{equation}
    \expectation \left( \sum_{i=1}^{n} \sum_{k=1}^{k_c} \sum_{k'=1}^{k_s} X_i \right)
    = \expectation \left( \sum_{i=1}^{n} \sum_{k=1}^{k_c} \sum_{k'=1}^{k_s} Y_i \right)
    = \sum_{i=1}^{n} \sum_{k=1}^{k_c} \sum_{k'=1}^{k_s} \expectation \left( Y_i \right) \text{.}
  \end{equation}
  Since $Y_i$ is a Bernoulli variable,
  \begin{multline}
    \expectation (Y_i) = \Pr (Y_i = 1)
    = \Pr \left( n\, k_c\, k_s \
    \max \left(
    \begin{split}
    \min_{0 \leq k < k_c}I_c (C_i, k)^2 \\
    \min_{0 \leq k' < k_s} I_s (C_i, k')^2
    \end{split}
    \right)  < \eps \right) =\\
    = \sum_{l=0}^{\infty} \Pr \left( n\, k_c\, k_s
    \max \left(
    \begin{split}
    \min_{0 \leq k < k_c}I_c (C_i, k)^2 \\
    \min_{0 \leq k' < k_s} I_s (C_i, k')^2
    \end{split}
    \right)  < \eps \ \Big|\ L_i=l
    \right)
    \cdot \Pr (L_i=l) \text{.}
  \end{multline}
  Let us finally denote by $\alpha_1 \dots \alpha_l$ the $l$ independent values of $|Du|$ and $\gamma_1 \dots \gamma_{l/s}$ the $l/s$ independent values of $|R_s|$.
  Again, we have assumed that $L_i$ is independent of the gradient and regularity distributions in the image. Thus conditionally to $L_i = l$,
  \begin{multline}
    \Pr \left( n\, k_c\, k_s
    \max \left(
    \begin{split}
    \min_{0 \leq k < k_c} I_c (C_i, k)^2 \\
    \min_{0 \leq k' < k_s} I_s (C_i, k')^2
    \end{split}
    \right) < \eps \ |\ L_i=l \right) = \\
    = \Pr \left( n\, k_c\, k_s
    \max \left(
    \begin{split}
    \min_{0 \leq k < k_c} I_c (C_i, k)^2 \\
    \min_{0 \leq k' < k_s} I_s (C_i, k')^2
    \end{split}
    \right) < \eps \right) = \\
    = \Pr \left(
    \max \left(
    \begin{split}
    \min_{0 \leq k < k_c} I_c (C_i, k) \\
    \min_{0 \leq k' < k_s} I_s (C_i, k')
    \end{split}
    \right) < \left( \frac{\eps}{n\, k_c\, k_s} \right)^{1 / 2} \right) = \\
    = \Pr \left( \min_{0 \leq k < k_c}I_c (C_i, k) < \left( \frac{\eps}{n\, k_c\, k_s} \right)^{1 / 2} \right) \cdot \\
    \Pr \left( \min_{0 \leq k' < k_s}I_s (C_i, k') < \left( \frac{\eps}{n\, k_c\, k_s} \right)^{1 / 2} \right) \text{.}
  \end{multline}
  From proof of Proposition~\ref{prop:nfaContrastedCurve_k},
  \begin{multline}
    \Pr \left( \min_{0 \leq k < k_c}I_c (C_i, k) < \left( \frac{\eps}{n\, k_c\, k_s} \right)^{1 / 2} \right) \cdot \\
    \Pr \left( \min_{0 \leq k' < k_s}I_s (C_i, k') < \left( \frac{\eps}{n\, k_c\, k_s} \right)^{1 / 2} \right) \leq \\
    \leq \left( \frac{\eps}{n\, k_c\, k_s} \right)^{1 / 2} \left( \frac{\eps}{n\, k_c\, k_s} \right)^{1 / 2} = \frac{\eps}{n\, k_c\, k_s} \textbf{.}
  \end{multline}
  Finally
  \begin{equation}
    \expectation (Y_i) \leq \frac{\eps}{n\, k_c\, k_s} \quad \Rightarrow \quad \sum_{i=1}^{n} \sum_{k=1}^{k_c} \sum_{k'=1}^{k_s} \expectation (Y_i) \leq \eps \text{.}
  \end{equation}
  
\end{proof}
